Actionable Neural Representations: Grid Cells from Minimal Constraints

To afford flexible behaviour, the brain must build internal representations that mirror the structure of variables in the external world. For example, 2D space obeys rules: the same set of actions combine in the same way everywhere (step north, then south, and you won't have moved, wherever you start). We suggest the brain must represent this consistent meaning of actions across space, as it allows you to find new short-cuts and navigate in unfamiliar settings. We term this representation an `actionable representation'. We formulate actionable representations using group and representation theory, and show that, when combined with biological and functional constraints - non-negative firing, bounded neural activity, and precise coding - multiple modules of hexagonal grid cells are the optimal representation of 2D space. We support this claim with intuition, analytic justification, and simulations. Our analytic results normatively explain a set of surprising grid cell phenomena, and make testable predictions for future experiments. Lastly, we highlight the generality of our approach beyond just understanding 2D space. Our work characterises a new principle for understanding and designing flexible internal representations: they should be actionable, allowing animals and machines to predict the consequences of their actions, rather than just encode.

==> Old_Wrtiting/Captions.tex <==
\textbf{A: Representation-Task Correspondence} A dataset $\{a_i,b_i\}$ (the crosses) must be classified linearly into the orange and green category. This cannot be done without changing the representation to include a third axis, $a^2 + b^2$. This includes no extra information but permits linear classification.

==> Old_Wrtiting/Conc_Old.tex <==
In this work we proposed a novel optimisation problem for neural representations. This optimisation problem was built using three ideas: first, the variable should be usefully encoded in the representation, different inputs should be represented differently; second, it should be representable using a set of neurons with positive bounded firing rates; third, the representation should be manipulable, allowing you to plan and make inferences internally.

We studied this objective and showed that the resulting optimal representations of 2D space are a good model for the entorhinal grid system. This allowed us to explain many observed features normatively, and to make predictions for novel aspects of the grid code, such as the size of a module from its tuning curve, and the relative angular alignment of modules. It is hoped that this theory can be widely applied to understand grid cell phenomena. 

==> Old_Wrtiting/LittleSnippets.tex <==
Finally, a very impressive body of work has convincingly shown that the grid cell system emerges mechanistically from a set of continuous attractor networks (CANs) (\cite{burak2009accurate}, \cite{gardner2022toroidal}). Our theory is situated one layer of abstraction higher than this. However, it is possible to see the combination of the structural and biological components of our objective as equivalent to being implemented by a CAN, and hence to see our work as optimising a representation under the constraint that it is implementable in a CAN. This link is described in section~\ref{sec:CANs}.

\section{Link to Continuous Attractor Networks}\label{sec:CANs}

The structural component of our normative objective is a proposal that the animal should be able to update its representation internally. For mathematical convenience, this is performed linearly in our framework. However extensive work has shown that in the entorhinal system the mechanistic underpinnings of just such an internal updating mechanism are CANs. CANs are a dynamical model of a neural circuit with a manifold of attractor points. Each attractor point corresponds to the encoding of a single input, and a velocity input is used to update the representation based on the movements (real or imagined) of the animal.

We must then wonder if there are links between these two ways of updating a representation. Here, we outline an argument that constraining the neural code using our structural and biological constraints play an equivalent role to asking that the underlying circuit be a CAN. This gives our normative theory a plausible mechanistic implementation.

In a CAN the neural dynamics evolve as follows:

\begin{equation}
    \tau \frac{d\vg}{dt} + \vg = \phi(\vW \vg)
\end{equation}

where $\vg$ is the vector of firing rates, $\vW$ is the recurrent weight connectivity, $\phi$ a pointwise nonlinearity, and $\tau$ a neuronal time constant. The defining feature of a CAN is its attractor manifold, a set of $N$ stable points of the dynamics ($N$ = number of neurons). For example, for encoding a 1D variable you can choose the dynamics to have N stable points:

\begin{equation}\label{eq:CAN_Stable}
    \vg(\theta_n) = \phi(\vW\vg(\theta_n)) \qquad \forall n = 1, \cdots, N
\end{equation}

What neural response profiles, $\vg(\theta)$, does this equation imply? 

Influenced by our previous analysis we will consider this in frequency space. Since the neural responses are evaluated at only 

\begin{enumerate}
    \item In N discrete, equally-spaced, samples the only possible frequencies present are those below the Nyquist frequency, which is half the sampling rate. Therefore, since points are sampled with a rate of $\frac{N}{2\pi}$ per radian, the nyquist angular frequency is $\frac{N}{2}$.
    \item Since the frequencies must be periodic, and hence integers, that means the code must contain a grid of only $\frac{N}{2}$ equally spaced frequencies. Further, the code must be positive in order to satisfy the non-linearity in equation~\ref{eq:CAN_Stable}. This matches our previous claims.
    \item However, previously on a circle we claimed that the code was a combination of any grid of frequencies, not just the lowest $\frac{N}{2}$. Fortunately, this can be fixed. We get to choose the mapping from the true variable to the encoded one, as long as when the true variable returns to its start value so does the encoded one. This means that the encoded variable can be twice, or any integer multiple of, the true one, since that just means while the true variable performs one loop round the circle, the encoded one does more than one. Therefore the grid code is made from a grid of frequencies with any base frequency, combined together to make a positive code. This is exactly like we claimed in our original argument.
    \item Finally we can extend this to the representation of a variable on a line. This is the same as before but now the mapping from the true variable to the encoded variable on the ring can be any multiple, since there is no periodicity requirement. Hence any grid will do, and the separation loss just selects which grid is optimal.
    \item In some sense this is a justification of the encoding schemes of \cite{stemmler2015connecting}, \cite{wei2015principle}, \cite{sreenivasan2011grid}, which assume grids then argue for their properties. In this work we have given two related arguments, one using CANs the other using representation theory, for why this is a reasonable starting point. From there we have largely agreed and extended the findings of these papers.
\end{enumerate}

==> Old_Wrtiting/OldLitReview.tex <==
Building and understanding neural representations through the principles they optimise is a staple of both Theoretical Neuroscience and Machine Learning. On the neuroscience side, classic work has argued that representations should maximise the information they convey about natural stimuli \cite{attneave1954some}, \cite{barlow1961possible}, and this has been broadly influential \cite{simoncelli2001natural} (fly visual: \cite{laughlin1981simple}, retinal: \cite{smirnakis1997adaptation}, or auditory: \cite{rieke1995naturalistic}). Similarly, visual representations have been analysed as sparse `independent components' encoding the visual scene, \cite{hyvarinen2010statistical}, \cite{olshausen1996emergence}. Relatedly, biological constraints, like positive firing rates \cite{sengupta2018manifold}, energy constraints \cite{niven2007fly}, or wiring minimisation \cite{hyvarinen2001topographic}, can play a key roles in producing particular representations. Our work takes inspiration from these approaches, but aims at a less sensory representation those presented here.

On the other hand, deep learning has revolutionised machine learning by learning task relevant representations. In the pursuit of clever representational objectives machine learners have reached far and wide \cite{bengio2013representation}. We are, for example, heavily influence by the work on equivariant representations. There are symmetries in the world, move a dog up and it is still a dog, and a classifier that assumes these are often easier to train. Cite leCun. Cite Taco Cohen. Maybe include something on plannable representations.

We are indebted to previous theoretical work on grid cells that can be roughly split into two categories. The first argue on decoding grounds that grid cells are a very efficient way to represent position, and that, among all possible grids, hexagons are optimal (\cite{mathis2012optimal}, \cite{mathis2012resolution}, \cite{sreenivasan2011grid}, \cite{wei2015principle}). These works are insightful, and make interesting predictions about the structure of the grid code, such as the relative lattice lengthscale in \cite{wei2015principle}. Indeed, our functional principle, that different positions should be represented maximally differently, is very similar in spirit to these decoding approaches. As such, we often reach similar conclusions, and we suspect that some of our novel results, such as the matching of the grid code to the room geometry, could have been derived by these authors. However, these works assume a grid tuning curve and either describe its properties or optimise over possible grids. Here, in contrast, we give a normative explanations of why choose a grid in the first place, allowing us to explain features like the alignment of grid axes within a module, which are detrimental from a pure decoding view \cite{stemmler2015connecting}. Further, our framing of the problem makes some analysis easier, and opens the possibility of fairly unlimited numerical exploration. As such, it could prove the most flexible framework in which to pursue future experimental predictions.

The second body of grid cell theory has focused on ideas of path integration, similar to our actionable principle. For example, some authors train a recurrent neural network to path integrate and show the resulting representations look like grid cells (\cite{cueva2018emergence}, \cite{banino2018vector}, \cite{sorscher2019unified}). The interpretation of these results has recently been clouded as the emergence of grid cells appears to be highly parameter dependent (\cite{schaeffer2022free}). We seek to add some clarity to this debate by providing a mathematical formalisation of a particular type of path-integrable representation, and showing why path-integrability combined with biological and functional constraints encourages the formation of multiple modules of grid cells. Our approach is most related to two papers that ask for path integration to be performed linearly, among other things, and show that grid cells emerge as a result (\cite{whittington2020tolman}, \cite{gao2021path}). In fact, our work can be seen as extracting from each of these the key elements necessary for a hexagonal grid code to be optimal.


==> Old_Wrtiting/Old_Predictions_Section.tex <==
\subsection{Module Relations}\label{sec:ModuleRelations}

It is very natural to ask what is the optimal arrangement of modules. How many modules should there be? How many neurons should belong to each module? What lattice should each module use?

\begin{figure}[h!]
\includegraphics[width=0.8\textwidth]{SketchFigures/Fig6ModRel.png}
\centering
\caption{}
\end{figure}

PLANNED PARAGRAPHS:

\begin{enumerate}
    \item The number of modules is simply a tradeoff between the number of neurons and sigma. Figure 6
    \item The angle between modules should be roughly 4 degrees, and appears to be. Figure 6. The lengthscales should be non-harmonically tuned. FINALISE MORE.
    \item I don't have a good way to think about the number of neurons in each module. I will try and get one.
\end{enumerate}

\subsection{Module Sizes from Data}\label{sec:ModuleSize}

As more neurons are included in a particular module the number of frequencies contributing to that module's receptive field increases. This causes the grid peaks to sharpen, figure 7A. This can be formalised and used to show that the number of neurons in a particular module, $N$, is proportional to the ratio of the grid lattice length to the grid peak width, appendix~\ref{app:Lattice-to-Peak}. In 2D the same argument applies but $N$ is proportional to the same ratio squared. This is intuitively sensible, when there are many neurons each can concentrate on encoding a smaller proportion of the inputs. This makes a prediction for the number of grid cells in a particular module based on the receptive field.

\begin{figure}[h!]
\includegraphics[width=0.8\textwidth]{SketchFigures/Fig7ModSize.png}
\centering
\caption{}
\end{figure}

This is a hard prediction to verify since you cannot measure the number of neurons in a particular module. You can, however, assume that in experiments each module is equally sampled, and therefore use the number of neurons measured in each module as a proxy for the total number. We tried this analysis with data from Stensola and found a degree of correlation between the receptive field properties and the number of measured neurons, figure 7B.

\subsection{Effect of Room Size}\label{sec:Room}

\begin{figure}[h!]
\includegraphics[width=0.8\textwidth]{SketchFigures/Fig8Room.png}
\centering
\caption{}
\end{figure}

There have been some curious findings about the way the grid code changes in different environments. For example, grid cells seem to align in particular ways to square rooms (Stensola 2015), figure 8A, and when changing from a square to a rectangular room some grids shift while others stay the same (Stensola 2012), figure 8B. These effects can be analysed in our framework by changing the distribution on points to reflect room geometry, for example this is the loss to study if the animal uniformly explores a square room of sidelength $L$:

\begin{equation}\mathcal{L} = \int_0^L\int_0^L e^{-\frac{|\vg(\vx) - \vg(\vx')|^2}{2\sigma^2}} |\vx - \vx'|^2 d\vx d\vx'\end{equation}

The effect of this change can be analysed to first order, appendix~\ref{app:Room}, and shown to introduce more complicated frequency biases. For example, certain frequencies whose wavelengths are integer multiples of the room size become preferred in square rooms, figure 8C. This can explain the alignment to room edges as an effect of the frequency biases, further it makes a prediction that the angle between grid and room should be largest for grids of the longest lengthscale, which we verify in data, figure 9C.

Finally, changing the room from a square to a rectangle again changes the optimal frequencies, figure 9D. If we assume that grid cells always choose to move to the optimal frequency nearest to them then we can explain some of the otherwise strange effects normatively, figure 9D. 


==> Old_Wrtiting/abstract_pel.tex <==


\peld{How should the brain build representations of the world?} Many \peld{relevant} variables \pel{in the world} have structure that can be behaviourally exploited, and \pel{the brain should build representations that make use of that} \peld{this} structure\peld{ should be mirrored in the variable's representation}. \pelc{not sure mine is better; feel free to ignore.} For example, navigating 2D space \peld{(or indeed, many more abstract spaces)} is easy because it obeys rules\peld{. No}\pel{: no} matter where you are\pel{,} you \pel{can} choose from an identical set of actions, and those actions combine in the same way everywhere \pel{(for instance,}\peld{:} step north\peld{,} \pel{and then} then south, and you won't have moved\pel{)}. This consistent meaning of actions across space is what allows you to find a new short-cut, or navigate in an unfamiliar setting. We hypothesise that animals \peld{should} have `actionable representations' in which actions have similarly consistent meaning, allowing us to predict our next position having taken any action from any position, even if we've never experienced this combination. We use group theory to formulate an optimisation problem over actionable representations\pel{,} and apply it to \peld{describe} the brain's encoding of 2D position. We show with analytic justification \pelc{strange phrase. can you just say ``we show analytially''? or is that too strong?} that the resulting optimal representations look like the empirically observed multiple modules of grid cells\pel{,} and \pel{we} provide deep \pel{is deep intuition different from intuition? ;)} intuition for this result. Further, we make a series of predictions about grid cells that compare favourably with data, explaining past observations normatively and making testable \peld{claims} \pel{predictions} for future experiments. Our work characterises a new, broadly applicable, principle with which to understand and design flexible internal representations: they should be actionable, allowing animals and machines to think, rather than just encode.
